ChemDIRT: A Diversified Instruction, Representation, and Task Benchmark for Robust Chemistry-LLM Evaluation

The rapid advancement of large language models (LLMs) has led to increasing interest in their application to scientific domains such as chemistry. However, existing chemistry benchmarks often provide only a narrow view of model capability, focusing on limited task sets while overlooking robustness to variations in problem formulation and chemical representation. As a result, reported performance may overestimate a model's true ability to reason consistently across realistic settings. To address this challenge, we introduce ChemDIRT (Diversified Instruction, Representation, and Task Benchmark), a comprehensive evaluation framework designed to assess the robustness of chemical reasoning in LLMs. ChemDIRT systematically measures model performance across variations in instructions and molecular representations while spanning eight categories of chemistry tasks. By evaluating both accuracy and consistency under these controlled perturbations, ChemDIRT provides a more reliable assessment of model reasoning capabilities than conventional single-format benchmarks. We benchmark a diverse set of open- and closed-source LLMs, revealing substantial prompt sensitivity, representation dependence, and uneven performance across task families.

==> body/6_app.tex <==
\section{Appendix}

%\subsection{Related Works Taxonomized}

%To verify the capabilities of chemistry models, it becomes necessary to construct meaningful benchmarks that reflect the domain-specific challenges of chemistry. Tests to measure the structure, symbolic, and experimental knowledge of chemistry LLMs are required to gauge its chemistry-specific reasoning. These chemistry tasks can broadly be categorized into eight categories, as previously defined. See Table \ref{tab:bench_stats} for the categorization of benchmarks according to task type.

%\subsubsection{Descriptive}

%A descriptive task is one where the model is asked to determine surface-level chemical information from structured or unstructured data (text, images, or graphs). These tasks involve elemental and structures recognition and labeling and do not require any inference beyond the presented data. These tasks serve as an assessment of the model's domain knowledge rather than any specific reasoning capability. They form a foundational layer necessary for enabling higher-level reasoning in chemistry.

%Descriptive tasks are those such as identifying features of a molecule, such as elements, ions, and functional groups, or determining the number or presence of atoms, rings, electrons, or isomers \cite{ChemistryQA, mirza2025framework, runcie2025assessing, li2025beyond, krallinger2015chemdner, hao2025can, yang2025r1}. Sometimes, the model may also be asked to match a molecule to a label description or vice versa \cite{zhang2024chemllm, guo2023can}, although these descriptions must contain only elemental or structural information, otherwise it belongs in the analytical category.

%\subsubsection{Classification}

%Classification tasks are among the most widely studied problem within the field of machine learning for chemistry and materials science. In these tasks, models are asked to predict categorical or binary chemical properties of molecules based on structures, often represented by a SMILES string. Foundational prediction benchmarks are from MoleculeNet, which is a collection of over 700,000 compounds tested on a range of different properties \cite{wu2018moleculenet}. The collection includes datasets such as HIV (experimentally measured ability to inhibit HIV replication), BBBP (blood-brain barrier penetration), and Tox21 (toxicity measurements on 12 biological targets). Several work have adapted these tasks for the LLM setting \cite{guo2023can, yu2024llasmol, zhong2025benchmarking, zhu2025moltextnet}.

%\subsubsection{Design}

%Design tasks require a model to generate or modify molecular structures given certain design parameters, such as similarity to another molecule or chemical properties. Examples of design tasks include molecular optimization, inverse design, and conditional or unconditional generation. In contrast to classification tasks which infer properties from molecules, design tasks generate molecules that match a set of characteristics.

%For unconditional generation, models aim to generate novel and chemically diverse molecules within a given data distribution. Common datasets to use are ZINC15 \cite{sterling2015zinc}, GuacaMol \cite{brown2019guacamol}, and MOSES \cite{polykovskiy2020molecular}, which evaluate generative quality across metrics including novelty, diversity, and synthesizability. Conditioned generation and inverse design tasks specify design objectives such as property constraints or molecular similarity, Mol-Instructions contains formatted prompts for description-guided molecular generation and optimization \cite{fang2023mol}. ChemRAG-Bench incorporates a subset of synthesis questions from Mol-Instructions, such as for description-based generation \cite{zhong2025benchmarking}. ChemLLMBench includes similar tasks for description-based generation, constructed from the ChEBI database \cite{guo2023can, degtyarenko2007chebi}. MolQA is a benchmark that similarly contains molecular descriptions for design \cite{liu2024multimodal}.

%Another design task include translating molecules between their SMILES, IUPAC, and chemical formulas \cite{ChemistryQA, sorokina2021coconut, narayanan2025training, mirza2025framework, fang2023mol, yu2024llasmol, guo2023can}. The philosophy behind this task matches conditional generation in that the model is prompted to generate a molecule based on a prior condition, i.e. the target written in a different line notation nomenclature.

%\subsubsection{Analytical}

%Analytical tasks form the broadest type of qualitative reasoning task. These tasks require models to interpret chemical knowledge and reason about causal outcomes. Unlike classification or design tasks, which can be solved using structural understanding and pattern recognition, analytical tasks require the ability to both recall and extrapolate from knowledge found across diverse domains of chemistry. General-purpose reasoning benchmarks such as MMLU and MMLU-pro include chemistry subsets that test conceptual understanding through multiple-choice questions \cite{hendrycks2020measuring, wang2024mmlu}. Analytical task benchmarks can target college \cite{mirza2025framework} and graduate school-level questions \cite{rein2024gpqa, du2025supergpqa}. Other analytical tasks include RAG question answering \cite{wellawatte2025chemlit}, molecular property analysis \cite{ma2025general}, hypothesis generation \cite{yang2024moose}, and biomedical research question answering \cite{jin2019pubmedqa}. Together, these benchmarks highlight the breadth and complexity of analytical reasoning in chemistry, positioning it as a key frontier for future development in domain-specific LLMs. In general, analytical type tasks can be thought of as non-numeric Q/A.

%\subsubsection{Regression}

%Regression tasks focus on estimating the continuous-valued molecular or material properties of a substance. Often, though not always, these numeric values are determined through real-world experimentation. Predicting quantum physical properties is a common regression task, with the QM9 dataset being a key representative \cite{ruddigkeit2012enumeration}. A similar dataset is the Open Catalyst 2022 (OC22) dataset, focusing on force and energy calculations \cite{tran2023open}. Other regression datasets include FreeSolv \cite{mobley2014freesolv}, ESOL, and Lipo \cite{wu2018moleculenet}. These prediction tasks have been adapted to the LLM setting \cite{yu2024llasmol, fang2023mol, zhong2025benchmarking, zhu2025moltextnet}.

%\subsubsection{Computational}

%Computational tasks are those that require arithmetic calculation, statistical analysis, and mathematical reasoning to arrive at numeric answers. These tasks often resemble mathematical word problems, but are based on chemical principles. Standard computational tasks are calculating moles, mass, concentration, pH, molarity, pressure, and temperature \cite{ChemistryQA}. Other tasks include yield prediction \cite{zhong2025benchmarking}, SAR analysis \cite{runcie2025assessing}, NMR spectroscopy \cite{runcie2025assessing}, graph/table analysis \cite{hao2025can, yang2025r1}, and stoichiometry \cite{valenti2024chemalgebra}. Given the wide range of computational tasks, several datasets specifically aggregate questions according to academic difficulty, ranging from elementary/secondary \cite{ma2025general}, collegiate \cite{hendrycks2020measuring, wang2024mmlu, wang2023scibench, mirza2025framework}, and graduate-levels questions \cite{rein2024gpqa, du2025supergpqa}.

%\subsubsection{Mechanistic}

%Mechanistic tasks require the model to explain or predict the underlying processes that drive chemical transformations. This reasoning often focuses on the movement of electrons, electric charge, and other stepwise processes. Answering these questions requires physical chemical knowledge and the ability to perform multi-step problem solving, addressing the "how" and "why" of chemical reactions.

%One of the largest corpora of chemical reaction information is found in the Open Reaction Database (ORD) \cite{kearnes2021open}. ORD is centralized data repository for sharing organic reaction data using an open-access schema. The schema provides a way to represent reaction details in a structured way. One of the largest datasets within ORD is the literature extracted reactions from the USPTO \cite{Lowe2017}. The USPTO is a common source for reaction datasets \cite{schneider2016s, coley2017prediction, jin2017predicting, chen2020retro, chen2024large, yuan2025uspto}. To streamline extraction and preprocessing from ORD and USPTO, ORDerly was introduced \cite{wigh2024orderly}. ORDerly also provides benchmarks for forward reaction prediction, retrosynthesis planning, and reaction condition prediction tasks. Beyond ORD, commercial data services such as Reaxys and SciFinder provide large-scale reaction data for mechanistic reaction modeling \cite{lawson2014making, gabrielson2018scifinder}. Other mechanistic tasks include product and solvent prediction \cite{zhang2024chemllm, ChemistryQA, runcie2025assessing}, forward reaction prediction \cite{guo2023can, liu2024multimodal, li2025beyond}, retrosynthesis \cite{li2025beyond}, and electron transfer prediction \cite{hao2025can}.

%\subsubsection{Relational}

%Relational tasks are by definition comparative, looking at the differences between molecules' structures, properties, and use-cases. Very few existing benchmarks consider relational tasks for LLM evaluation. However, ChemLLMBench \cite{guo2023can} includes reagent selection, formulated as a ranking problem, as a relational task. ChemBench4K \cite{zhang2024chemllm} also includes a selection task where the most similar molecule out of four candidates to a given description must be chosen.

\subsection{Subset Splits}

In Table \ref{tab:subset_split_full}, we present the full details on the number of data examples per subtask. We further denote if the dataset is created by ourselves or sampled, in part or in whole, from another data source.

\input{tables/subset_split_full}

%\subsection{Regression Quantization}

%We have four regression tasks, each of which have had their label values binned into label ranges. For ESOL, a label value $\geq$ 0 is "highly soluble", a value in the range of [-2, 0) is "soluble", one in the range of [-4, -2) is "slightly soluble", and any label value $<$ -4 is "insoluble" \cite{sorkun2019aqsoldb}. For lipophilicity, [1, 3] is "optimal", $>$ 3 is "highly lipophilic",  and $<$ 1 is "hydrophilic/lipophobic" \cite{waring2010lipophilicity}. FreeSolv follows the standard thermodynamic understanding of solvation, so negative values indicate "favorable transfer" into water, and positive values show "unfavorable transfer" \cite{tokmakoff2021concepts}. For O$_2$ permeability, values must be non-negative. Values between [0, 1) represent barrer values less than that of S100-0.3, values between [1, 10) represent barrer values between that of S100-0.3 and Nafion 212, and $\geq$ 10 represents barrer greater than that of Nafion 212. With each label value being associated to categories, these become the label values for the modified evaluation.

%\subsection{Prompt Templates}

%We include the prompt templates for each of our included subtasks.

%\input{tables/prompts_all}

\subsection{Benchmark Statistics}

Table \ref{tab:bench_stats} displays information other benchmark datasets for chemistry, including dataset counts and the type of tasks from our taxonomy represented.

\input{tables/bench_stats}

%\input{tables/bench_results_alt_metrics}

==> tables/bench_reason.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{||l|c|c|c|c|c|c|c||}
    \hline
        \multirow{2}{*}{}
        & \multicolumn{1}{c|}{Descriptive}
        & \multicolumn{3}{c|}{Qualitative}
        & \multicolumn{2}{c|}{Quantitative}
        & \multicolumn{1}{c||}{Mechanistic} \\
        & & Classification & Design & Analytical & Regression & Computational & \\
        \hline \hline
        MoleculeNet \cite{wu2018moleculenet} & & \checkmark & & & \checkmark & & \\
        QM9 \cite{ruddigkeit2012enumeration} & & & \checkmark & & \checkmark & & \\
        ZINC15 \cite{sterling2015zinc} & & & \checkmark & & & & \\
        GuacaMol \cite{brown2019guacamol} & & & \checkmark & & & & \\
        MOSES \cite{polykovskiy2020molecular} & & & \checkmark & & & & \\
        ORDerly \cite{wigh2024orderly} & & & & & & & \checkmark \\
        ChemLit-QA \cite{wellawatte2025chemlit} & & & & \checkmark & & & \\
        TOMATO-Chem \cite{yang2024moose} & & & & \checkmark & & & \\
        PubMedQA \cite{jin2019pubmedqa} & & & & \checkmark & & & \\
        SciBench \cite{wang2023scibench} & & & & & & \checkmark & \\
        ChemAlgebra \cite{valenti2024chemalgebra} & & & & & & \checkmark & \\
        MMK12 \cite{ma2025general} & & & & \checkmark & & \checkmark & \\
        MMLU \cite{hendrycks2020measuring} & & & & \checkmark & & \checkmark & \\
        MMLU-Pro \cite{wang2024mmlu} & & & & \checkmark & & \checkmark & \\
        GPQA \cite{rein2024gpqa} & & & & \checkmark & & \checkmark & \\
        SuperGPQA \cite{du2025supergpqa} & & & & \checkmark & & \checkmark & \\
        MolQA \cite{liu2024multimodal} & & & \checkmark & \checkmark & & & \\
        MolPair \cite{liu2024multimodal} & & & \checkmark & & & & \checkmark \\
        COCONUT \cite{sorokina2021coconut} & & & \checkmark & & & & \\
        SMolInstruct \cite{yu2024llasmol} & & \checkmark & \checkmark & & \checkmark & & \checkmark \\
        ChemistryQA \cite{ChemistryQA} & \checkmark & & \checkmark & & & \checkmark & \checkmark \\
        ChemIQ \cite{runcie2025assessing} & \checkmark & & & & & \checkmark & \checkmark \\
        EMMA \cite{hao2025can} & \checkmark & & & & & \checkmark & \checkmark \\
        R1-Onevision-Bench \cite{yang2025r1} & \checkmark & & & & & \checkmark & \\
        ChemBench \cite{mirza2025framework} & \checkmark & & \checkmark & \checkmark & & \checkmark & \\
        ChemCoTBench \cite{li2025beyond} & \checkmark & & & & & & \checkmark \\
        ChemRAG-Bench \cite{zhong2025benchmarking} & \checkmark & & \checkmark & & \checkmark & & \\
        Mol-Instructions \cite{fang2023mol} & \checkmark & & \checkmark & \checkmark & \checkmark & & \\
        ChemLLMBench \cite{guo2023can} & \checkmark & \checkmark & \checkmark & & & & \checkmark \\
        ChemBench4K \cite{zhang2024chemllm} & \checkmark & & & & \checkmark & \checkmark & \checkmark \\
        MolTextNet \cite{zhu2025moltextnet} & \checkmark & \checkmark & & & \checkmark & & \\
        \hline
    \end{tabular}
    }
    \caption{The type of reasoning tasks each benchmark is evaluating.}
    \label{tab:bench_reason}
\end{table*}



==> tables/bench_results.tex <==
\begin{sidewaystable*}
    \centering
    \vspace*{0.8\textheight}
    \begin{adjustbox}{width=\textheight,center}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \hline
            %Model & Task &&&&&&&&&&&&&&&&&&&&&&&&&&&& \\
            %\hline
            \multirow{2}{*}{Model}

                & \multicolumn{4}{c|}{Descriptive}
                & \multicolumn{4}{c|}{Classification}
                & \multicolumn{3}{c|}{Design}
                & \multicolumn{5}{c|}{Analytical}\\
                \cline{2-17}
                & Carbon Count & Ring Count & Functional Group & Bond Type & BACE & BBBP & ClinTox & HIV & IUPAC2SMILES & SMILES2IUPAC & Text-Description Design & RAG-Based QA & True/False w/Explanation & Open Response & Molecule Captioning & \\
            \hline \hline
            ChemLLM &&&&&&&&&&&&&&&& \\
            ChemDFM &&&&&&&&&&&&&&&& \\
            Chemr &&&&&&&&&&&&&&&& \\
            General-Reasoner &&&&&&&&&&&&&&&& \\
            Ether0 &&&&&&&&&&&&&&&& \\
            Falcon &&&&&&&&&&&&&&&& \\
            Galatica &&&&&&&&&&&&&&&& \\
            Qwen2 &&&&&&&&&&&&&&&& \\
            Qwen3 &&&&&&&&&&&&&&&& \\
            Mistral &&&&&&&&&&&&&&&& \\
            Gemma2 &&&&&&&&&&&&&&&& \\
            Gemma3 &&&&&&&&&&&&&&&& \\
            Llama2 &&&&&&&&&&&&&&&& \\
            Llama3 &&&&&&&&&&&&&&&& \\
            Deepseek-r1 &&&&&&&&&&&&&&&& \\
            GPT-4o &&&&&&&&&&&&&&&& \\
            GPT-4.1 &&&&&&&&&&&&&&&& \\
            GPT-5 &&&&&&&&&&&&&&&& \\
            \hline
        \end{tabular}
    \end{adjustbox}

    \vspace*{12pt}

    \begin{adjustbox}{width=\textheight,center}
        \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
            \hline
            %Model & Task &&&&&&&&&&&&&&&&&&&&&&&&&&&& \\
            %\hline
            \multirow{2}{*}{Model}
                & \multicolumn{4}{c|}{Regression}
                & \multicolumn{4}{c|}{Computational}
                & \multicolumn{2}{c|}{Mechanistic}
                & \multicolumn{3}{c|}{Relational} \\
                \cline{2-14}
                & ESOL & Lipo & FreeSolv & Oxygen Permeability & & Coefficient Balancing & Yield Prediction & & Forward Prediction & Retrosynthesis Planning & Representation Equivalence & Chemical Similarity & Molar Weight \\
            \hline \hline
            ChemLLM &&&&&&&&&&&&& \\
            ChemDFM &&&&&&&&&&&&& \\
            Chemr &&&&&&&&&&&&& \\
            General-Reasoner &&&&&&&&&&&&& \\
            Ether0 &&&&&&&&&&&&& \\
            Falcon &&&&&&&&&&&&& \\
            Galatica &&&&&&&&&&&&& \\
            Qwen2 &&&&&&&&&&&&& \\
            Qwen3 &&&&&&&&&&&&& \\
            Mistral &&&&&&&&&&&&& \\
            Gemma2 &&&&&&&&&&&&& \\
            Gemma3 &&&&&&&&&&&&& \\
            Llama2 &&&&&&&&&&&&& \\
            Llama3 &&&&&&&&&&&&& \\
            Deepseek-r1 &&&&&&&&&&&&& \\
            GPT-4o &&&&&&&&&&&&& \\
            GPT-4.1 &&&&&&&&&&&&& \\
            GPT-5 &&&&&&&&&&&&& \\
            \hline
        \end{tabular}
    \end{adjustbox}
    \caption{Baseline Model Evaluation on Benchmark}
    \label{tab:bench_results}
\end{sidewaystable*}


==> tables/bench_results_alt_metrics.tex <==
\begin{table*}
    \centering
    \caption{Baseline Model Evaluation on Benchmark. The best open-source model is \textbf{bold}. The second best is \underline{underlined}.}
    \label{tab:bench_results}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|
        ccc|ccc|ccc|
        ccc|ccc|ccc|ccc|}
        \hline
        \multirow{3}{*}{Model}
        & \multicolumn{9}{c|}{Design}
        & \multicolumn{12}{c|}{Analytical} \\
        \cline{2-22}
        & \multicolumn{3}{c|}{IUPAC2SMILES}
        & \multicolumn{3}{c|}{SMILES2IUPAC}
        & \multicolumn{3}{c|}{Desc-Based Gen}
        & \multicolumn{3}{c|}{RAG-Based QA}
        & \multicolumn{3}{c|}{TF w/ Explanation}
        & \multicolumn{3}{c|}{Open Response}
        & \multicolumn{3}{c|}{Captioning} \\
        \cline{2-22}
        & Morgans & BLEU & ROUGE & EM & BLEU & ROUGE & EM & BLEU & ROUGE & EM & BLEU & ROUGE & EM & BLEU & ROUGE & EM & BLEU & ROUGE & EM & BLEU & ROUGE \\
        \hline \hline
        ChemLLM & 0.0934 & \textbf{0.4013} & 0.0664 & 0.2684 & 0.0157 & 0.1055 & \underline{0.3130} &&&&&&&&&&&&&& \\
        ChemDFM & \textbf{0.5783} & 0.0709 & \textbf{0.7168} & 0.5088 & 0.0149 & 0.1022 & \textbf{0.4132} &&&&&&&&&&&&&& \\
        Chemr & 0.3167 & \underline{0.3981} & 0.4603 & 0.1757 & 0.0205 & 0.0995 & 0.3149 &&&&&&&&&&&&&& \\
        General-Reasoner & 0.1111 & 0.0531 & 0.0000 & \textbf{0.5790} & 0.0246 & 0.1028 & 0.1626 &&&&&&&&&&&&&& \\
        Ether0 & \underline{0.4289} & 0.0987 & \textbf{0.5334} & 0.1588 & 0.0134 & 0.0980 & 0.0712 &&&&&&&&&&&&&& \\
        Falcon & 0.0153 & 0.0412 & 0.0185 & 0.4838 & \underline{0.0325} & 0.0864 & 0.1934 &&&&&&&&&&&&&& \\
        Galatica & 0.0098 & 0.0000 & 0.0000 & 0.2261 & 0.0288 & 0.0976 & 0.0402 &&&&&&&&&&&&&& \\
        Qwen2 & 0.0823 & 0.1997 & 0.0728 & \underline{0.5286} & 0.0281 & 0.1125 & 0.1898 &&&&&&&&&&&&&& \\
        Qwen3 & 0.0592 & 0.0490 & 0.0353 & 0.2516 & 0.0213 & 0.1147 & 0.1800 &&&&&&&&&&&&&& \\
        Mistral & 0.0572 & 0.1136 & 0.0252 & 0.4828 & 0.0172 & \underline{0.1295} & 0.2186 &&&&&&&&&&&&&& \\
        Gemma2 & 0.0079 & 0.0052 & 0.0000 & 0.4318 & 0.0225 & 0.0822 & 0.0892 &&&&&&&&&&&&&& \\
        Gemma3 & 0.1117 & 0.2090 & 0.0356 & 0.2960 & 0.0189 & 0.1246 & 0.2027 &&&&&&&&&&&&&& \\
        Llama2 & 0.0357 & 0.0379 & 0.0350 & 0.2232 & 0.0250 & 0.1027 & 0.1118 &&&&&&&&&&&&&& \\
        Llama3 & 0.1332 & 0.1484 & 0.0722 & 0.2481 & \textbf{0.0333} & \textbf{0.1457} & 0.1956 &&&&&&&&&&&&&& \\
        Deepseek-r1 & 0.0460 & 0.0421 & 0.0423 & 0.2778 & 0.0199 & 0.1094 & 0.1448 &&&&&&&&&&&&&& \\
        \hline
        Claude-4.5 & 0.1935 & 0.1337 & 0.5028 & 0.6761 & 0.0208 & 0.1425 & 0.1021 &&&&&&&&&&&&&& \\
        GPT-4o & 0.5148 & 0.4781 & 0.4807 & 0.4328 & 0.1499 & 0.1420 & 0.1261 &&&&&&&&&&&&&& \\
        GPT-4.1 & 0.5831 & 0.5017 & 0.5347 & 0.5046 & 0.1682 & 0.1738 & 0.1027 &&&&&&&&&&&&&& \\
        GPT-5 & 0.4256 & 0.3282 & 0.4861 & 0.3206 & 0.1739 & 0.1780 & 0.0785 &&&&&&&&&&&&&& \\
        \hline
    \end{tabular}
    }
\end{table*}

\begin{table*}
    \clearpage
    \ContinuedFloat

    \newpage

    \vspace{12pt}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|
        ccc|ccc|ccc|ccc|}
        \hline
        \multirow{3}{*}{Model}
        & \multicolumn{12}{c|}{Mechanistic} \\
        \cline{2-13}
        & \multicolumn{3}{c|}{Forward (S)}
        & \multicolumn{3}{c|}{Forward (F)}
        & \multicolumn{3}{c|}{Retro (S)}
        & \multicolumn{3}{c|}{Retro (F)} \\
        \cline{2-13}
        & EM & BLEU & ROUGE & EM & BLEU & ROUGE & EM & BLEU & ROUGE & EM & BLEU & ROUGE \\
        \hline \hline
        ChemLLM & 0.2657 & 0.2437 & 0.3643 & 0.2153 & 0.5100 & 0.4300 & \underline{0.5600} &&&& \\
        ChemDFM & \textbf{0.5689} & 0.3186 & \underline{0.4238} & 0.3806 & \underline{0.6300} & 0.4000 & 0.5100 \\
        Chemr & \underline{0.5738} & 0.1923 & \textbf{0.4652} & 0.2646 & 0.4800 & 0.5400 & 0.5400 \\
        General-Reasoner & 0.2395 & 0.2685 & 0.3458 & 0.3159 & \textbf{0.6400} & 0.5100 & 0.4900 \\
        Ether0 & 0.3622 & 0.3048 & 0.4169 & \textbf{0.5070} & 0.5300 & 0.4900 & 0.5100 \\
        Falcon & 0.1305 & \underline{0.4673} & 0.1108 & 0.1794 & 0.5100 & 0.3900 & 0.5700 \\
        Galatica & 0.0242 & 0.0001 & 0.0422 & 0.0010 & 0.4800 & 0.4100 & \underline{0.5600} \\
        Qwen2 & 0.1719 & 0.2792 & 0.2195 & 0.3471 & 0.4400 & 0.4700 & 0.5400 \\
        Qwen3 & 0.1976 & 0.3341 & 0.2387 & \underline{0.3984} & 0.5300 & \textbf{0.5800} & 0.5100 \\
        Mistral & 0.1753 & 0.2952 & 0.2042 & 0.3149 & 0.5200 & \underline{0.5500} & 0.5000 \\
        Gemma2 & 0.2425 & \textbf{0.5649} & 0.2570 & 0.3548 & 0.4400 & 0.4800 & \textbf{0.6000} \\
        Gemma3 & 0.2162 & 0.3397 & 0.2225 & 0.2596 & 0.4900 & 0.5400 & 0.5300 \\
        Llama2 & 0.1889 & 0.4569 & 0.2319 & 0.3348 & 0.5800 & 0.4800 & 0.4200 \\
        Llama3 & 0.2321 & 0.3885 & 0.1592 & 0.3554 & 0.5200 & 0.5200 & 0.5100 \\
        Deepseek-r1 & 0.2244 & 0.3651 & 0.2815 & 0.3356 & 0.5500 & 0.5300 & 0.3600 \\
        \hline
        Claude-4.5 & 0.4126 & 0.1642 & 0.5147 & 0.3620 & 0.7500 & 0.6100 & 0.5400  \\
        GPT-4o & 0.4349 & 0.4494 & 0.4340 & 0.3925 & 0.7100 & 0.6200 & 0.8200 \\
        GPT-4.1 & 0.4807 & 0.5090 & 0.4734 & 0.4006 & 0.8400 & 0.6400 & 0.8700 \\
        GPT-5 & 0.7699 & 0.2345 & 0.5083 & 0.4042 & 0.8400 & 0.6300 & 0.9100 \\
        \hline
    \end{tabular}
    }
\end{table*}


==> tables/bench_results_new.tex <==
\begin{table*}
    \centering
    \caption{Baseline Model Evaluation on Benchmark. The best open-source model is \textbf{bold}. The second best is \underline{underlined}.}
    \label{tab:bench_results}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|cccc|cccc|}
\hline
\multirow{2}{*}{Model}
& \multicolumn{4}{c|}{Descriptive}
& \multicolumn{4}{c|}{Classification} \\
\cline{2-9}

& Carbon Count
& Ring Count
& Functional Group
& Bond Type
& BACE
& BBBP
& ClinTox
& HIV \\
\hline \hline

ChemLLM & 0.0400 & 0.2600 & 0.3200 & 0.3400 & 0.5197 & 0.1569 & 0.5946 & \textbf{0.9500} \\
ChemDFM & \textbf{0.1600} & 0.2300 & 0.4800 & 0.4400 & \textbf{0.8158} & \underline{0.6569} & 0.6351 & \underline{0.9000} \\
Chemr & 0.0500 & \underline{0.3900} & 0.5100 & 0.4600 & 0.5066 & 0.3235 & 0.8446 & 0.8300 \\
General-Reasoner & 0.0900 & \textbf{0.4500} & 0.0700 & 0.0700 & 0.4342 & 0.1569 & 0.8581 & 0.3400 \\
Ether0 & \underline{0.1000} & 0.2500 & 0.5100 & 0.4600 & \underline{0.5987} & 0.3333 & 0.5878 & 0.8200 \\
Falcon & 0.0300 & 0.2000 & 0.4900 & 0.3900 & 0.4342 & \textbf{0.8431} & 0.5068 & 0.0500 \\
Galatica & 0.0200 & 0.0800 & 0.3400 & 0.3000 & 0.5197 & 0.4706 & 0.5541 & 0.5400 \\
Qwen2 & 0.0700 & 0.2500 & 0.5300 & 0.5300 & 0.5197 & 0.1569 & 0.2500 & 0.5200 \\
Qwen3 & 0.0500 & 0.3000 & \textbf{0.6000} & \underline{0.5400} & 0.4934 & 0.1961 & 0.8041 & \textbf{0.9500} \\
Mistral & 0.0500 & 0.2500 & 0.3600 & 0.3800 & 0.4803 & 0.3922 & 0.4662 & 0.4500 \\
Gemma2 & 0.0800 & 0.1900 & 0.4600 & 0.4900 & 0.5000 & 0.1765 & 0.4257 & \textbf{0.9500} \\
Gemma3 & 0.0700 & 0.2200 & 0.4800 & 0.4900 & 0.5197 & 0.1667 & 0.5743 & 0.6600 \\
Llama2 & 0.0400 & 0.1300 & 0.2500 & 0.2500 & 0.4408 & 0.2843 & 0.5878 & 0.8000 \\
Llama3 & 0.0300 & 0.1300 & 0.4000 & 0.3900 & 0.4737 & 0.3627 & 0.7027 & 0.3600 \\
Deepseek-r1 & 0.0400 & 0.3200 & \underline{0.5500} & \textbf{0.5500} & 0.4737 & 0.2549 & 0.7432 & \textbf{0.9500} \\
\hline
Claude-4.5 & 0.4300 & 0.9400 & 0.6600 & 0.8000 & 0.3510 & 0.5714 & 0.8581 & 0.9500 \\
GPT-4o & 0.1000 & 0.6000 & 0.7800 & 0.5000 & 0.4868 & 0.4118 & 0.5270 & 0.6100 \\
GPT-4.1 & 0.3400 & 0.6500 & 0.7700 & 0.5800 & 0.5066 & 0.4706 & 0.4706 & 0.6200 \\
GPT-5 & 0.9000 & 0.9500 & 0.8500 & 0.9500 & 0.4403 & 0.4825 & 0.8316 & 0.7600 \\
\hline

\end{tabular}
    }

    \vspace*{12pt}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|ccc|ccc|ccc|ccc|ccc|}
    \hline
    \multirow{2}{*}{Model}
    & \multicolumn{3}{c|}{IUPAC$\rightarrow$SMILES}
    & \multicolumn{3}{c|}{SMILES$\rightarrow$IUPAC}
    & \multicolumn{3}{c|}{Photo$\rightarrow$SMILES}
    & \multicolumn{3}{c|}{Photo$\rightarrow$IUPAC}
    & \multicolumn{3}{c|}{Description-Based} \\
    \cline{2-16}

    & Valid & MACCS & Morgan
    & Valid & MACCS & Morgan
    & Valid & MACCS & Morgan
    & Valid & MACCS & Morgan
    & Valid & MACCS & Morgan \\
    \hline \hline

    ChemLLM          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    ChemDFM          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Chemr            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    General-Reasoner & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Ether0           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Falcon           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Galatica         & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen2            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen3            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Mistral          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Gemma2           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Gemma3           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Llama2           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Llama3           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Deepseek-r1      & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    \hline
    Claude-4.5
    & 0.407$\pm$0.234 & 0.534$\pm$0.199 & 0.431$\pm$0.170
    & 1.000$\pm$0.000 & 0.017$\pm$0.008 & 0.014$\pm$0.007
    & -- & -- & --
    & -- & -- & --
    & -- & -- & -- \\

    GPT-4o
    & 0.613$\pm$0.036 & 0.510$\pm$0.009 & 0.202$\pm$0.007
    & 1.000$\pm$0.000 & 0.204$\pm$0.062 & 0.088$\pm$0.025
    & -- & -- & --
    & -- & -- & --
    & -- & -- & -- \\

    GPT-4.1
    & 0.630$\pm$0.084 & 0.576$\pm$0.005 & 0.269$\pm$0.008
    & 0.998$\pm$0.005 & 0.323$\pm$0.031 & 0.150$\pm$0.010
    & -- & -- & --
    & -- & -- & --
    & -- & -- & -- \\

    GPT-5
    & 0.515$\pm$0.060 & 0.586$\pm$0.010 & 0.273$\pm$0.004
    & 1.000$\pm$0.000 & 0.207$\pm$0.023 & 0.095$\pm$0.013
    & -- & -- & --
    & -- & -- & --
    & -- & -- & -- \\

    \hline

    \end{tabular}
    }
\end{table*}

\begin{table*}[t]
\centering
\caption{Performance on analytical tasks.}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|cccc|cccc|cccc|}
\hline
\multirow{2}{*}{Model}
& \multicolumn{4}{c|}{RAG-Based QA}
& \multicolumn{4}{c|}{TF w/ Explanation}
& \multicolumn{4}{c|}{Open Response} \\
\cline{2-13}

& EM & BLEU & ROUGE & METEOR
& EM & BLEU & ROUGE & METEOR
& EM & BLEU & ROUGE & METEOR \\
\hline \hline

ChemLLM & 0.1327 & 0.0000 & 0.5333 & 0.5184 & 0.0400 & 0.0000 & 0.0400 & 0.0200 & 0.0400 & 0.0000 & 0.1315 & 0.1107 \\
ChemDFM & 0.1991 & 0.0000 & 0.6125 & 0.5783 & 0.0400 & 0.0000 & 0.0400 & 0.0200 & 0.0600 & 0.0000 & 0.1357 & 0.1148 \\
Chemr & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
General-Reasoner & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Ether0 & 0.1327 & 0.0000 & 0.4660 & 0.4607 & 0.0200 & 0.0000 & 0.0200 & 0.0100 & 0.0400 & 0.0000 & 0.0746 & 0.0619 \\
Falcon & 0.1280 & 0.0000 & 0.5348 & 0.5035 & 0.0100 & 0.0000 & 0.0100 & 0.0050 & 0.0500 & 0.0000 & 0.1382 & 0.1142 \\
Galatica & 0.1801 & 0.0000 & 0.6136 & 0.5900 & 0.0500 & 0.0000 & 0.0500 & 0.0250 & 0.0600 & 0.0000 & 0.1761 & 0.1577 \\
Qwen2 & 0.1564 & 0.0000 & 0.5689 & 0.5485 & 0.1100 & 0.0000 & 0.1100 & 0.0550 & 0.0500 & 0.0000 & 0.1307 & 0.1086 \\
Qwen3 & 0.1185 & 0.0000 & 0.5253 & 0.5383 & 0.1100 & 0.0000 & 0.1100 & 0.0550 & 0.0600 & 0.0000 & 0.1259 & 0.1006 \\
Mistral & 0.1232 & 0.0000 & 0.5212 & 0.4995 & 0.1000 & 0.0000 & 0.1000 & 0.0500 & 0.0500 & 0.0000 & 0.1306 & 0.1195 \\
Gemma2 & 0.1564 & 0.0000 & 0.5526 & 0.5272 & 0.0200 & 0.0000 & 0.0200 & 0.0100 & 0.0500 & 0.0000 & 0.1417 & 0.1201 \\
Gemma3 & 0.1801 & 0.0000 & 0.6077 & 0.5778 & 0.0500 & 0.0000 & 0.0500 & 0.0250 & 0.0900 & 0.0000 & 0.2176 & 0.1912 \\
Llama2 & 0.1754 & 0.0000 & 0.5813 & 0.5480 & 0.0400 & 0.0000 & 0.0400 & 0.0200 & 0.0500 & 0.0000 & 0.1302 & 0.1179 \\
Llama3 & 0.1422 & 0.0000 & 0.5241 & 0.5075 & 0.0200 & 0.0000 & 0.0200 & 0.0100 & 0.0500 & 0.0000 & 0.1478 & 0.1312 \\
Deepseek-r1 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\hline
Claude-4.5 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
GPT-4o & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
GPT-4.1 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
GPT-5 & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\hline

\end{tabular}
}
\label{tab:analytical_results}
\end{table*}

\begin{table*}
    \clearpage
    \ContinuedFloat

    \newpage

    \caption{Baseline Model Evaluation on Benchmark (cont.)}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|cccc|cc|cc|cc|cc|}
    \hline
    \multirow{3}{*}{Model}
    & \multicolumn{4}{c|}{Regression}
    & \multicolumn{8}{c|}{Computational} \\
    \cline{2-13}

    & ESOL
    & Lipo
    & FreeSolv
    & O$_2$ Permeability
    & \multicolumn{2}{c|}{Unit Calculation}
    & \multicolumn{2}{c|}{Coefficient Balancing}
    & \multicolumn{2}{c|}{Yield Prediction}
    & \multicolumn{2}{c|}{Molar Weight} \\
    \cline{6-13}

    &
    &
    &
    &
    &
    RMSE & Rel.
    & RMSE & Rel.
    & RMSE & Rel.
    & RMSE & Rel. \\
    \hline \hline

    ChemLLM          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    ChemDFM          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Chemr            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    General-Reasoner & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Ether0           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Falcon           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Galatica         & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen2            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen3            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Mistral          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Gemma2           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Gemma3           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Llama2           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Llama3           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Deepseek-r1      & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    \hline
    Claude-4.5       & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    GPT-4o           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    GPT-4.1          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    GPT-5            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    \hline

    \end{tabular}
    }

    \vspace{12pt}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|ccc|cccc|ccc|cccc|}
    \hline
    \multirow{2}{*}{Model}
    & \multicolumn{3}{c|}{Forward (SMILES)}
    & \multicolumn{4}{c|}{Forward (Formula)}
    & \multicolumn{3}{c|}{Retrosynthesis (SMILES)}
    & \multicolumn{4}{c|}{Retrosynthesis (Formula)} \\
    \cline{2-15}

    & Valid & MACCS & Morgan
    & Valid & EM & Cosine & F1
    & Valid & MACCS & Morgan
    & Valid & EM & Cosine & F1 \\
    \hline \hline

    ChemLLM          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    ChemDFM          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Chemr            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    General-Reasoner & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Ether0           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Falcon           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Galatica         & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen2            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Qwen3            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Mistral          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Gemma2           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Gemma3           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Llama2           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Llama3           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    Deepseek-r1      & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    \hline
    Claude-4.5       & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    GPT-4o           & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    GPT-4.1          & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    GPT-5            & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
    \hline

\end{tabular}
}
\end{table*}

\begin{table*}[t]
\centering
\caption{Performance on relational reasoning tasks (accuracy).}
\resizebox{\textwidth}{!}{
\begin{tabular}{|c|ccc|ccc|ccc|}
\hline
\multirow{2}{*}{Model}
& \multicolumn{3}{c|}{Forward (Photo)}
& \multicolumn{3}{c|}{Retrosynthesis (Photo)}
& \multicolumn{3}{c|}{Relational} \\
\cline{2-10}

& Valid & MACCS & Morgan
& Valid & MACCS & Morgan
& Rep. Eq.
& Chem. Sim.
& Weight Comp. \\
\hline \hline

ChemLLM          & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
ChemDFM          & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Chemr            & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
General-Reasoner & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Ether0           & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Falcon           & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Galatica         & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Qwen2            & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Qwen3            & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Mistral          & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Gemma2           & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Gemma3           & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Llama2           & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Llama3           & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
Deepseek-r1      & -- & -- & -- & -- & -- & -- & -- & -- & -- \\
\hline
Claude-4.5
& 0.758$\pm$0.420 & 0.010$\pm$0.002 & 0.000$\pm$0.000
& 0.533$\pm$0.517 & 0.013$\pm$0.002 & 0.000$\pm$0.000
& -- & -- & -- \\

GPT-4o
& 0.388$\pm$0.238 & 0.009$\pm$0.001 & 0.000$\pm$0.000
& 0.300$\pm$0.128 & 0.013$\pm$0.004 & 0.000$\pm$0.000
& -- & -- & -- \\

GPT-4.1
& 0.203$\pm$0.116 & 0.011$\pm$0.003 & 0.000$\pm$0.000
& 0.218$\pm$0.126 & 0.014$\pm$0.002 & 0.000$\pm$0.000
& -- & -- & -- \\

GPT-5
& 0.543$\pm$0.131 & 0.017$\pm$0.013 & 0.003$\pm$0.007
& 0.705$\pm$0.369 & 0.021$\pm$0.011 & 0.003$\pm$0.007
& -- & -- & -- \\
    \hline

\end{tabular}
}
\label{tab:relational_results}
\end{table*}

==> tables/bench_results_old.tex <==
\begin{table*}
    \centering
    \caption{Baseline Model Evaluation on Benchmark. The best open-source model is \textbf{bold}. The second best is \underline{underlined}.}
    \label{tab:bench_results}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        %Model & Task &&&&&&&&&&&&&&&&&&&&&&&&&&&& \\
        %\hline
        \multirow{2}{*}{Model}

            & \multicolumn{4}{c|}{Descriptive (Acc)}
            & \multicolumn{4}{c|}{Classification (Acc)} \\
            \cline{2-9}
            & Carbon Count & Ring Count & Functional Group & Bond Type & BACE & BBBP & ClinTox & HIV \\
        \hline \hline
        ChemLLM & 0.0400 & 0.2600 & 0.3200 & 0.3400 & 0.5197 & 0.1569 & 0.5946 & \textbf{0.9500} \\
        ChemDFM & \textbf{0.1600} & 0.2300 & 0.4800 & 0.4400 & \textbf{0.8158} & \underline{0.6569} & 0.6351 & \underline{0.9000} \\
        Chemr & 0.0500 & \underline{0.3900} & 0.5100 & 0.4600 & 0.5066 & 0.3235 & 0.8446 & 0.8300 \\
        General-Reasoner & 0.0900 & \textbf{0.4500} & 0.0700 & 0.0700 & 0.4342 & 0.1569 & 0.8581 & 0.3400 \\
        Ether0 & \underline{0.1000} & 0.2500 & 0.5100 & 0.4600 & \underline{0.5987} & 0.3333 & 0.5878 & 0.8200 \\
        Falcon & 0.0300 & 0.2000 & 0.4900 & 0.3900 & 0.4342 & \textbf{0.8431} & 0.5068 & 0.0500 \\
        Galatica & 0.0200 & 0.0800 & 0.3400 & 0.3000 & 0.5197 & 0.4706 & 0.5541 & 0.5400 \\
        Qwen2 & 0.0700 & 0.2500 & 0.5300 & 0.5300 & 0.5197 & 0.1569 & 0.2500 & 0.5200 \\
        Qwen3 & 0.0500 & 0.3000 & \textbf{0.6000} & \underline{0.5400} & 0.4934 & 0.1961 & 0.8041 & \textbf{0.9500} \\
        Mistral & 0.0500 & 0.2500 & 0.3600 & 0.3800 & 0.4803 & 0.3922 & 0.4662 & 0.4500 \\
        Gemma2 & 0.0800 & 0.1900 & 0.4600 & 0.4900 & 0.5000 & 0.1765 & 0.4257 & \textbf{0.9500} \\
        Gemma3 & 0.0700 & 0.2200 & 0.4800 & 0.4900 & 0.5197 & 0.1667 & 0.5743 & 0.6600 \\
        Llama2 & 0.0400 & 0.1300 & 0.2500 & 0.2500 & 0.4408 & 0.2843 & 0.5878 & 0.8000 \\
        Llama3 & 0.0300 & 0.1300 & 0.4000 & 0.3900 & 0.4737 & 0.3627 & 0.7027 & 0.3600 \\
        Deepseek-r1 & 0.0400 & 0.3200 & \underline{0.5500} & \textbf{0.5500} & 0.4737 & 0.2549 & 0.7432 & \textbf{0.9500} \\
        \hline
        Claude-4.5 & 0.4300 & 0.9400 & 0.6600 & 0.8000 & 0.3510 & 0.5714 & 0.8581 & 0.9500 \\
        GPT-4o & 0.1000 & 0.6000 & 0.7800 & 0.5000 & 0.4868 & 0.4118 & 0.5270 & 0.6100 \\
        GPT-4.1 & 0.3400 & 0.6500 & 0.7700 & 0.5800 & 0.5066 & 0.4706 & 0.4706 & 0.6200 \\
        GPT-5 & 0.9000 & 0.9500 & 0.8500 & 0.9500 & 0.4403 & 0.4825 & 0.8316 & 0.7600 \\
        \hline
    \end{tabular}
    }

    \vspace*{12pt}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        %Model & Task &&&&&&&&&&&&&&&&&&&&&&&&&&&& \\
        %\hline
        \multirow{2}{*}{Model}
            & \multicolumn{3}{c|}{Design (Morgans / BLEU)}
            & \multicolumn{4}{c|}{Analytical (ROUGE)}\\
            \cline{2-8}
            & IUPAC2SMILES & SMILES2IUPAC & Desc-Based Gen & RAG-Based QA & TF w/Explanation & Open Response & Captioning \\
        \hline \hline
        ChemLLM & 0.0934 & \textbf{0.4013} & 0.0664 & 0.2684 & 0.0157 & 0.1055 & \underline{0.3130} \\
        ChemDFM & \textbf{0.5783} & 0.0709 & \textbf{0.7168} & 0.5088 & 0.0149 & 0.1022 & \textbf{0.4132} \\
        Chemr & 0.3167 & \underline{0.3981} & 0.4603 & 0.1757 & 0.0205 & 0.0995 & 0.3149 \\
        General-Reasoner & 0.1111 & 0.0531 & 0.0000 & \textbf{0.5790} & 0.0246 & 0.1028 & 0.1626 \\
        Ether0 & \underline{0.4289} & 0.0987 & \textbf{0.5334} & 0.1588 & 0.0134 & 0.0980 & 0.0712 \\
        Falcon & 0.0153 & 0.0412 & 0.0185 & 0.4838 & \underline{0.0325} & 0.0864 & 0.1934 \\
        Galatica & 0.0098 & 0.0000 & 0.0000 & 0.2261 & 0.0288 & 0.0976 & 0.0402 \\
        Qwen2 & 0.0823 & 0.1997 & 0.0728 & \underline{0.5286} & 0.0281 & 0.1125 & 0.1898 \\
        Qwen3 & 0.0592 & 0.0490 & 0.0353 & 0.2516 & 0.0213 & 0.1147 & 0.1800 \\
        Mistral & 0.0572 & 0.1136 & 0.0252 & 0.4828 & 0.0172 & \underline{0.1295} & 0.2186 \\
        Gemma2 & 0.0079 & 0.0052 & 0.0000 & 0.4318 & 0.0225 & 0.0822 & 0.0892 \\
        Gemma3 & 0.1117 & 0.2090 & 0.0356 & 0.2960 & 0.0189 & 0.1246 & 0.2027 \\
        Llama2 & 0.0357 & 0.0379 & 0.0350 & 0.2232 & 0.0250 & 0.1027 & 0.1118 \\
        Llama3 & 0.1332 & 0.1484 & 0.0722 & 0.2481 & \textbf{0.0333} & \textbf{0.1457} & 0.1956 \\
        Deepseek-r1 & 0.0460 & 0.0421 & 0.0423 & 0.2778 & 0.0199 & 0.1094 & 0.1448 \\
        \hline
        Claude-4.5 & 0.1935 & 0.1337 & 0.5028 & 0.6761 & 0.0208 & 0.1425 & 0.1021 \\
        GPT-4o & 0.5148 & 0.4781 & 0.4807 & 0.4328 & 0.1499 & 0.1420 & 0.1261 \\
        GPT-4.1 & 0.5831 & 0.5017 & 0.5347 & 0.5046 & 0.1682 & 0.1738 & 0.1027 \\
        GPT-5 & 0.4256 & 0.3282 & 0.4861 & 0.3206 & 0.1739 & 0.1780 & 0.0785 \\
        \hline
    \end{tabular}
    }
\end{table*}

\begin{table*}
    \clearpage
    \ContinuedFloat

    \newpage

    \caption{Baseline Model Evaluation on Benchmark (cont.)}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
        \hline
        %Model & Task &&&&&&&&&&&&&&&&&&&&&&&&&&&& \\
        %\hline
        \multirow{2}{*}{Model}
            & \multicolumn{4}{c|}{Regression (Acc))}
            & \multicolumn{4}{c|}{Computational (Match-in-10 Acc)} \\
            \cline{2-9}
            & ESOL & Lipo & FreeSolv & O$_2$ Permeability & Unit Calculation & Coefficient Balancing & Yield Prediction & Molar Weight \\
        \hline \hline
        ChemLLM & 0.2389 & \textbf{0.5810} & 0.4923 & 0.0391 & 0.1393 & 0.3000 & 0.2300 & 0.0100 \\
        ChemDFM & 0.2035 & 0.5619 & \textbf{0.6769} & 0.0615 & \underline{0.1741} & 0.4700 & \textbf{0.4233} & 0.2000 \\
        Chemr & \underline{0.3451} & 0.1714 & 0.3692 & 0.2793 & 0.1045 & 0.2400 & 0.1700 & 0.0400 \\
        General-Reasoner & 0.2212 & 0.4381 & 0.4000 & 0.2346 & \textbf{0.2289} & 0.5100 & 0.2167 & \underline{0.2900} \\
        Ether0 & 0.1947 & 0.4952 & \underline{0.6308} & 0.0335 & 0.0846 & 0.5700 & 0.2200 & 0.1400 \\
        Falcon & 0.3274 & \underline{0.5714} & 0.6154 & 0.0112 & 0.0846 & 0.4300 & 0.0000 & 0.0200 \\
        Galatica & \textbf{0.3628} & 0.2095 & 0.4308 & 0.0056 & 0.1443 & 0.2600 & 0.0000 & 0.0100 \\
        Qwen2 & 0.1504 & 0.2762 & 0.4923 & \underline{0.2849} & 0.1542 & 0.4900 & 0.1200 & 0.0800 \\
        Qwen3 & 0.2920 & 0.2571 & 0.4154 & 0.1173 & 0.1741 & 0.3700 & 0.1100 & 0.0600 \\
        Mistral & 0.3097 & 0.2667 & 0.4769 & 0.0223 & 0.1343 & 0.5100 & 0.0067 & 0.0900 \\
        Gemma2 & \textbf{0.3628} & 0.1429 & 0.6000 & 0.0112 & 0.1692 & \textbf{0.6800} & 0.0067 & \textbf{0.4200} \\
        Gemma3 & 0.1947 & 0.2667 & 0.4615 & \textbf{0.2961} & 0.1144 & \underline{0.6100} & \underline{0.2533} & 0.1000 \\
        Llama2 & 0.2566 & 0.2476 & 0.5231 & 0.0615 & 0.1194 & 0.4700 & 0.0667 & 0.1200 \\
        Llama3 & 0.1947 & 0.2762 & 0.5538 & 0.1955 & 0.1592 & 0.5100 & 0.1167 & 0.0300 \\
        Deepseek-r1 & 0.2655 & 0.1810 & 0.5231 & 0.0503 & 0.1493 & 0.3800 & 0.0700 & 0.1100 \\
        \hline
        Claude-4.5 & 0.4159 & 0.5119 & 0.7538 & 0.3966 & 0.2920 & 0.7000 & 0.9367 & 0.9500 \\
        GPT-4o & 0.5929 & 0.5429 & 0.6923 & 0.3575 & 0.4726 & 0.4700 & 0.6900 & 0.5100 \\
        GPT-4.1 & 0.6283 & 0.4762 & 0.8000 & 0.3296 & 0.3284 & 0.5200 & 0.3900 & 0.6600 \\
        GPT-5 & 0.6195 & 0.5524 & 0.8000 & 0.3575 & 0.4826 & 0.8200 & 0.9333 & 0.8900 \\
        \hline
    \end{tabular}
    }

    \vspace{12pt}

    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c||c|}
        \hline
        %Model & Task &&&&&&&&&&&&&&&&&&&&&&&&&&&& \\
        %\hline
        \multirow{2}{*}{Model}
            & \multicolumn{4}{c|}{Mechanistic (Morgans / BLEU)}
            & \multicolumn{3}{c||}{Relational (Acc)}
            \\
            \cline{2-8}
            & Forward (S) & Forward (F) & Retrosynthesis (S) & Retrosynthesis (F) & Rep Equivalence & Chemical Similarity & Weight Comparison \\
        \hline \hline
        ChemLLM & 0.2657 & 0.2437 & 0.3643 & 0.2153 & 0.5100 & 0.4300 & \underline{0.5600}  \\
        ChemDFM & \textbf{0.5689} & 0.3186 & \underline{0.4238} & 0.3806 & \underline{0.6300} & 0.4000 & 0.5100 \\
        Chemr & \underline{0.5738} & 0.1923 & \textbf{0.4652} & 0.2646 & 0.4800 & 0.5400 & 0.5400 \\
        General-Reasoner & 0.2395 & 0.2685 & 0.3458 & 0.3159 & \textbf{0.6400} & 0.5100 & 0.4900 \\
        Ether0 & 0.3622 & 0.3048 & 0.4169 & \textbf{0.5070} & 0.5300 & 0.4900 & 0.5100 \\
        Falcon & 0.1305 & \underline{0.4673} & 0.1108 & 0.1794 & 0.5100 & 0.3900 & 0.5700 \\
        Galatica & 0.0242 & 0.0001 & 0.0422 & 0.0010 & 0.4800 & 0.4100 & \underline{0.5600} \\
        Qwen2 & 0.1719 & 0.2792 & 0.2195 & 0.3471 & 0.4400 & 0.4700 & 0.5400 \\
        Qwen3 & 0.1976 & 0.3341 & 0.2387 & \underline{0.3984} & 0.5300 & \textbf{0.5800} & 0.5100 \\
        Mistral & 0.1753 & 0.2952 & 0.2042 & 0.3149 & 0.5200 & \underline{0.5500} & 0.5000 \\
        Gemma2 & 0.2425 & \textbf{0.5649} & 0.2570 & 0.3548 & 0.4400 & 0.4800 & \textbf{0.6000} \\
        Gemma3 & 0.2162 & 0.3397 & 0.2225 & 0.2596 & 0.4900 & 0.5400 & 0.5300 \\
        Llama2 & 0.1889 & 0.4569 & 0.2319 & 0.3348 & 0.5800 & 0.4800 & 0.4200 \\
        Llama3 & 0.2321 & 0.3885 & 0.1592 & 0.3554 & 0.5200 & 0.5200 & 0.5100 \\
        Deepseek-r1 & 0.2244 & 0.3651 & 0.2815 & 0.3356 & 0.5500 & 0.5300 & 0.3600 \\
        \hline
        Claude-4.5 & 0.4126 & 0.1642 & 0.5147 & 0.3620 & 0.7500 & 0.6100 & 0.5400  \\
        GPT-4o & 0.4349 & 0.4494 & 0.4340 & 0.3925 & 0.7100 & 0.6200 & 0.8200 \\
        GPT-4.1 & 0.4807 & 0.5090 & 0.4734 & 0.4006 & 0.8400 & 0.6400 & 0.8700 \\
        GPT-5 & 0.7699 & 0.2345 & 0.5083 & 0.4042 & 0.8400 & 0.6300 & 0.9100 \\
        \hline
    \end{tabular}
    }
\end{table*}


==> tables/bench_results_summary.tex <==
\begin{table*}[t]
\centering
\label{tab:benchmark_summary}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline
\textbf{Model}
& \textbf{Description}
& \textbf{Classification}
& \textbf{Design}
& \textbf{Analytical}
& \textbf{Regression}
& \textbf{Computational}
& \textbf{Mechanistic}
& \textbf{Relational} \\
\hline\hline
ChemLLM & 0.2400 & 0.5553 & 0.1870 & 0.1757 & 0.3378 & 0.1698 & 0.2723 & 0.5000 \\
ChemDFM & 0.3275 & \textbf{0.7520} & \textbf{0.4553} & \textbf{0.2598} & \underline{0.3759} & \underline{0.3169} & \textbf{0.4230} & 0.5133 \\
Chemr & 0.3525 & \underline{0.6262} & \underline{0.3917} & 0.1527 & 0.2913 & 0.1386 & 0.3739 & 0.5200 \\
General-Reasoner & 0.1700 & 0.4473 & 0.0547 & \underline{0.2173} & 0.3235 & 0.3114 & 0.2924 & \textbf{0.5467} \\
Ether0 & 0.3300 & 0.5849 & 0.3537 & 0.0854 & 0.3386 & 0.2537 & \underline{0.3977} & 0.5100 \\
Falcon & 0.2775 & 0.4585 & 0.0250 & 0.1990 & \textbf{0.3814} & 0.1337 & 0.2218 & 0.4900 \\
Galactica & 0.1850 & 0.5211 & 0.0000 & 0.0982 & 0.2522 & 0.1036 & 0.0169 & 0.4833 \\
Qwen2 & 0.3450 & 0.3617 & 0.1183 & 0.2073 & 0.3009 & 0.2111 & 0.2544 & 0.4833 \\
Qwen3 & \textbf{0.3725} & 0.6109 & 0.0478 & 0.1419 & 0.2705 & 0.1785 & 0.2922 & \underline{0.5400} \\
Mistral & 0.2600 & 0.4472 & 0.0653 & 0.2120 & 0.2691 & 0.1853 & 0.2474 & 0.5233 \\
Gemma2 & 0.3050 & 0.5131 & 0.0000 & 0.1564 & 0.2792 & \textbf{0.3190} & 0.3548 & 0.5067 \\
Gemma3 & 0.3200 & 0.4802 & 0.1188 & 0.1606 & 0.3048 & 0.2694 & 0.2595 & 0.5200 \\
Llama2 & 0.1675 & 0.5282 & 0.0362 & 0.1241 & 0.2722 & 0.1940 & 0.3031 & 0.4933 \\
Llama3 & 0.2375 & 0.4748 & 0.1179 & 0.1550 & 0.3051 & 0.2040 & 0.2838 & 0.5167 \\
Deepseek-r1 & \underline{0.3675} & 0.6055 & 0.0435 & 0.1375 & 0.2550 & 0.1773 & 0.3017 & 0.4800 \\
\hline
Claude-4.5 & 0.7083 & 0.6826 & 0.2767 & 0.2354 & 0.5196 & 0.7197 & 0.3384 & 0.6333 \\
GPT-4o & 0.4950 & 0.5089 & 0.4912 & 0.2127 & 0.5464 & 0.5357 & 0.4277 & 0.7167 \\
GPT-4.1 & 0.5850 & 0.5170 & 0.5398 & 0.2366 & 0.5585 & 0.4746 & 0.4660 & 0.7833 \\
GPT-5 & 0.9125 & 0.6286 & 0.4133 & 0.1878 & 0.5824 & 0.7815 & 0.4792 & 0.7933 \\
\hline
\end{tabular}
}
\caption{Condensed benchmark results showing average performance across the eight task categories. Each entry is the unweighted average of tasks within the corresponding category. The best open-source model is \textbf{bold}. The second best is \underline{underlined}.}
\vspace{-6px}
\end{table*}


==> tables/chemdirt_stats.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{||l|c|c|c|c|c|}
            \hline
            & Size & Task Type & Task Count & Designed for LLMs & Chemistry-specific \\
            \hline \hline
            MoleculeNet \cite{wu2018moleculenet} & $\sim 700000$ & Classification/Regression & & No & Yes \\
            QM9 \cite{ruddigkeit2012enumeration} & $\sim 130000$ & Regression/Design & & No & Yes \\
            ZINC15 \cite{sterling2015zinc} & $> 20$ billion & Design & & No & Yes \\
            GuacaMol \cite{brown2019guacamol} & $\sim 1600000$ & Design & & No & Yes \\
            MOSES \cite{polykovskiy2020molecular} & $\sim 2000000$ & Design & & No & Yes \\
            ORDerly \cite{wigh2024orderly} & $\sim 1770000$ & Mechanistic & & No & Yes \\
            ChemLit-QA \cite{wellawatte2025chemlit} & $1054$ & Analytical & & Yes & Yes \\
            TOMATO-Chem \cite{yang2024moose} & $51$ & Analytical & & Yes & Yes \\
            PubMedQA \cite{jin2019pubmedqa} & $\sim 274000$ & Analytical & & Yes & No \\
            SciBench \cite{wang2023scibench} & $869$ & Computational & & Yes & No \\
            ChemAlgebra \cite{valenti2024chemalgebra} & $\sim 40000$ & Computational & & Yes & Yes \\
            MMK12 \cite{ma2025general} & $\sim 18000$ & Analytical/Computational & & Yes & No \\
            MMLU \cite{hendrycks2020measuring} & $\sim 14000$ & Analytical/Computational & & Yes & No \\
            MMLU-Pro \cite{wang2024mmlu} & $\sim 12000$ & Analytical/Computational & & Yes & No \\
            GPQA \cite{rein2024gpqa} & $448$ & Analytical/Computational & & Yes & No \\
            SuperGPQA \cite{du2025supergpqa} & $\sim 27000$ & Analytical/Computational & & Yes & No \\
            MolQA \cite{liu2024multimodal} & $\sim 11000$ & Design/Analytical & & Yes & Yes \\
            MolPair \cite{liu2024multimodal} & $\sim 300000$ & Design/Mechanistic & & Yes & Yes \\
            COCONUT \cite{sorokina2021coconut} & $\sim 820000$ & Descriptive & & No & Yes \\
            ChemistryQA \cite{ChemistryQA} & $500$ & Descriptive/Computational/Mechanistic & & Yes & Yes \\
            ChemIQ \cite{runcie2025assessing} & $816$ & Descriptive/Computational/Mechanistic & & Yes & Yes \\
            EMMA \cite{hao2025can} & $2778$ & Descriptive/Computational/Mechanistic & & Yes & No \\
            R1-Onevision-Bench \cite{yang2025r1} & $942$ & Descriptive/Computational & & Yes & No \\
            ChemBench \cite{mirza2025framework} & $2788$ & Descriptive/Analytical/Computational & & Yes & Yes \\
            ChemCoTBench \cite{li2025beyond} & $1495$ & Descriptive/Mechanistic & & Yes & Yes \\
            SMolInstruct \cite{yu2024llasmol} & $\sim 33000$ & Descriptive/Classification/Regression & & Yes & Yes \\
            ChemRAG-Bench \cite{zhong2025benchmarking} & $1932$ & Descriptive/Design/Regression & & Yes & Yes \\
            Mol-Instructions \cite{fang2023mol} & $\sim 2000000$ & Descriptive/Design/Analytical/Regression & & Yes & Yes \\
            ChemLLMBench \cite{guo2023can} & $800$ & Descriptive/Classification/Design/Mechanistic & & Yes & Yes \\
            ChemBench4K \cite{zhang2024chemllm} & $4100$ & Descriptive/Regression/Computational/Mechanistic & & Yes & Yes \\
            MolTextNet \cite{zhu2025moltextnet} & $\sim 2500000$ & Description/Classification/Regression & & Yes & Yes \\
            \hline
        \end{tabular}
    }
    \caption{More details on the chemistry benchmark tasks.}
    \label{tab:bench_stats}
\end{table*}



==> tables/multi_prompt_eval.tex <==
\begin{table*}[]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{||l|c|c|c|c|c|c|c||}
    \hline
        \multirow{2}{*}{}
        & \multicolumn{1}{c|}{Descriptive}
        & \multicolumn{3}{c|}{Qualitative}
        & \multicolumn{2}{c|}{Quantitative}
        & \multicolumn{1}{c||}{Mechanistic} \\
        & & Classification & Design & Analytical & Regression & Computational & \\
        \hline \hline
        MoleculeNet \cite{wu2018moleculenet} & & \checkmark & & & \checkmark & & \\
        QM9 \cite{ruddigkeit2012enumeration} & & & \checkmark & & \checkmark & & \\
        ZINC15 \cite{sterling2015zinc} & & & \checkmark & & & & \\
        GuacaMol \cite{brown2019guacamol} & & & \checkmark & & & & \\
        MOSES \cite{polykovskiy2020molecular} & & & \checkmark & & & & \\
        ORDerly \cite{wigh2024orderly} & & & & \checkmark & & & \checkmark \\
        ChemLit-QA \cite{wellawatte2025chemlit} & & & & \checkmark & & & \\
        TOMATO-Chem \cite{yang2024moose} & & & & \checkmark & & & \\
        PubMedQA \cite{jin2019pubmedqa} & & & & \checkmark & & & \\
        SciBench \cite{wang2023scibench} & & & & & & \checkmark & \\
        ChemAlgebra \cite{valenti2024chemalgebra} & & & & & & \checkmark & \\
        MMK12 \cite{ma2025general} & & & & \checkmark & & \checkmark & \\
        MMLU \cite{hendrycks2020measuring} & & & & \checkmark & & \checkmark & \\
        MMLU-Pro \cite{wang2024mmlu} & & & & \checkmark & & \checkmark & \\
        GPQA \cite{rein2024gpqa} & & & & \checkmark & & \checkmark & \\
        SuperGPQA \cite{du2025supergpqa} & & & & \checkmark & & \checkmark & \\
        MolQA \cite{liu2024multimodal} & & & \checkmark & \checkmark & & & \\
        MolPair \cite{liu2024multimodal} & & & & & & & \checkmark \\
        COCONUT \cite{sorokina2021coconut} & \checkmark & & & & & & \\
        ChemistryQA \cite{ChemistryQA} & \checkmark & & & & & \checkmark & \checkmark \\
        ChemIQ \cite{runcie2025assessing} & \checkmark & & & & & \checkmark & \checkmark \\
        EMMA \cite{hao2025can} & \checkmark & & & & & \checkmark & \checkmark \\
        R1-Onevision-Bench \cite{yang2025r1} & \checkmark & & & & & \checkmark & \\
        ChemBench \cite{mirza2025framework} & \checkmark & & & \checkmark & & \checkmark & \\
        ChemCoTBench \cite{li2025beyond} & \checkmark & & & & & & \checkmark \\
        SMolInstruct \cite{yu2024llasmol} & \checkmark & \checkmark & & & \checkmark & & \\
        ChemRAG-Bench \cite{zhong2025benchmarking} & \checkmark & & \checkmark & & \checkmark & & \\
        Mol-Instructions \cite{fang2023mol} & \checkmark & & \checkmark & \checkmark & \checkmark & & \\
        ChemLLMBench \cite{guo2023can} & \checkmark & \checkmark & \checkmark & & & & \checkmark \\
        ChemData \cite{zhang2024chemllm} & \checkmark & & & & \checkmark & \checkmark & \checkmark \\
        MolTextNet \cite{zhu2025moltextnet} & \checkmark & \checkmark & & & \checkmark & & \\
        \hline
    \end{tabular}
    }
    \caption{Performance of LLMs on the MolWeight task across different prompt formats.}
    \label{fig:multi_prompt_eval}
\end{table*}



==> tables/prompts_all.tex <==
\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Carbon Count Prompt Variants} \\
\midrule
Count the number of carbon atoms in \texttt{\{SMILES\}}. \\
How many carbons are present in the molecule \texttt{\{SMILES\}}? \\
Determine the total carbon count for \texttt{\{SMILES\}}. \\
Report the number of carbon atoms in \texttt{\{SMILES\}}. \\
For the SMILES \texttt{\{SMILES\}}, how many carbon atoms does it contain? \\
Compute the total number of carbons in \texttt{\{SMILES\}}. \\
Identify the carbon atom count in the molecule \texttt{\{SMILES\}}. \\
What is the total count of carbon atoms in \texttt{\{SMILES\}}? \\
Given \texttt{\{SMILES\}}, return the number of carbon atoms. \\
How many carbon atoms make up the structure \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{Carbon atom counting prompt templates.}
\label{tab:prompts_carbon}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Ring Count Prompt Variants} \\
\midrule
Count the number of rings in \texttt{\{SMILES\}}. \\
How many ring systems does \texttt{\{SMILES\}} contain? \\
Determine the ring count for \texttt{\{SMILES\}}. \\
Report the number of rings in the molecule \texttt{\{SMILES\}}. \\
For \texttt{\{SMILES\}}, how many distinct rings are present? \\
What is the total number of rings in \texttt{\{SMILES\}}? \\
Compute the ring count of \texttt{\{SMILES\}}. \\
How many cyclic structures are in \texttt{\{SMILES\}}? \\
Find the number of rings contained in \texttt{\{SMILES\}}. \\
Given the SMILES \texttt{\{SMILES\}}, return its ring count. \\
\bottomrule
\end{tabular}
\caption{Ring counting prompt templates.}
\label{tab:prompts_ring}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Functional Group Presence Prompt Variants} \\
\midrule
Does the molecule \texttt{\{SMILES\}} contain a \texttt{\{FG\}} functional group? \\
Is a \texttt{\{FG\}} group present in \texttt{\{SMILES\}}? \\
Determine whether \texttt{\{SMILES\}} includes a \texttt{\{FG\}} functional group. \\
Does \texttt{\{SMILES\}} have at least one \texttt{\{FG\}} group? \\
Check if the structure \texttt{\{SMILES\}} contains a \texttt{\{FG\}}. \\
For the molecule \texttt{\{SMILES\}}, is a \texttt{\{FG\}} functional group present? \\
Assess whether \texttt{\{SMILES\}} exhibits a \texttt{\{FG\}} group. \\
Does the SMILES \texttt{\{SMILES\}} encode a \texttt{\{FG\}} functional group? \\
Identify if \texttt{\{SMILES\}} contains a \texttt{\{FG\}}. \\
Is the \texttt{\{FG\}} functional group found in \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{Functional group presence prompt templates.}
\label{tab:prompts_fg}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Bond Type Presence Prompt Variants} \\
\midrule
Does the molecule \texttt{\{SMILES\}} contain any \texttt{\{BOND\}} bonds? \\
Are \texttt{\{BOND\}} bonds present in \texttt{\{SMILES\}}? \\
Determine whether \texttt{\{SMILES\}} includes at least one \texttt{\{BOND\}} bond. \\
Check if the structure \texttt{\{SMILES\}} has a \texttt{\{BOND\}} bond. \\
For the molecule \texttt{\{SMILES\}}, does a \texttt{\{BOND\}} bond exist? \\
Does \texttt{\{SMILES\}} feature any \texttt{\{BOND\}} bonds? \\
Assess whether \texttt{\{SMILES\}} contains a \texttt{\{BOND\}} bond type. \\
Is a \texttt{\{BOND\}} bond found in the SMILES \texttt{\{SMILES\}}? \\
Identify whether \texttt{\{SMILES\}} has any \texttt{\{BOND\}} bonds. \\
Does the chemical structure \texttt{\{SMILES\}} include \texttt{\{BOND\}} bonding? \\
\bottomrule
\end{tabular}
\caption{Bond type presence prompt templates.}
\label{tab:prompts_bond}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{BACE Classification Prompt Variants} \\
\midrule
Predict the BACE inhibitor property for the molecule with SMILES: \texttt{\{SMILES\}} \\
Is the compound represented by \texttt{\{SMILES\}} a BACE inhibitor? \\
Classify the molecule \texttt{\{SMILES\}} with respect to its BACE inhibitory activity. \\
Given the SMILES \texttt{\{SMILES\}}, determine if it has BACE inhibition properties. \\
Does the structure \texttt{\{SMILES\}} act as a BACE inhibitor? \\
Evaluate the BACE activity of the molecule encoded as \texttt{\{SMILES\}}. \\
For the molecule \texttt{\{SMILES\}}, return whether it is a BACE inhibitor or not. \\
From the SMILES \texttt{\{SMILES\}}, predict the binary BACE property. \\
Can you assess whether \texttt{\{SMILES\}} corresponds to a BACE inhibitor? \\
What is the BACE property classification for the compound \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{BACE classification prompt templates.}
\label{tab:prompts_bace}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{BBBP Classification Prompt Variants} \\
\midrule
Predict the blood-brain barrier penetration (BBBP) property for the molecule with SMILES: \texttt{\{SMILES\}} \\
Does the compound \texttt{\{SMILES\}} cross the blood-brain barrier? \\
Classify the molecule \texttt{\{SMILES\}} with respect to blood-brain barrier permeability. \\
Given the SMILES \texttt{\{SMILES\}}, determine if it penetrates the BBB. \\
Will the molecule \texttt{\{SMILES\}} be brain-penetrant? \\
Evaluate whether \texttt{\{SMILES\}} crosses the blood-brain barrier. \\
For the molecule \texttt{\{SMILES\}}, return if it has BBB permeability or not. \\
From the SMILES \texttt{\{SMILES\}}, predict the binary BBBP property. \\
Can you assess if \texttt{\{SMILES\}} penetrates the blood-brain barrier? \\
What is the BBBP classification for the compound \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{BBBP classification prompt template.}
\label{tab:prompts_bbbp}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{ClinTox Classification Prompt Variants} \\
\midrule
Predict the clinical trial toxicity outcome for the molecule with SMILES: \texttt{\{SMILES\}}. \\
Did the compound represented by \texttt{\{SMILES\}} fail clinical trials due to toxicity? \\
Classify the molecule \texttt{\{SMILES\}} with respect to clinical trial toxicity. \\
Given the SMILES \texttt{\{SMILES\}}, determine whether the compound exhibits clinical trial toxicity. \\
Does the structure \texttt{\{SMILES\}} indicate failure in clinical trials due to toxicity? \\
Evaluate the clinical trial toxicity of the molecule encoded as \texttt{\{SMILES\}}. \\
For the molecule \texttt{\{SMILES\}}, return whether it failed clinical trials because of toxicity. \\
From the SMILES \texttt{\{SMILES\}}, predict the binary clinical trial toxicity label. \\
Can you assess whether \texttt{\{SMILES\}} corresponds to a clinically toxic compound? \\
What is the clinical trial toxicity classification for the compound \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{Clinical trial toxicity classification prompt template.}
\label{tab:prompts_clintox}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{HIV Classification Prompt Variants} \\
\midrule
Predict the HIV inhibitor property for the molecule with SMILES: \texttt{\{SMILES\}} \\
Is the compound \texttt{\{SMILES\}} active against HIV? \\
Classify the molecule \texttt{\{SMILES\}} with respect to its HIV inhibitory activity. \\
Given the SMILES \texttt{\{SMILES\}}, determine if it has HIV inhibition properties. \\
Does the structure \texttt{\{SMILES\}} inhibit HIV? \\
Evaluate the HIV activity of the molecule encoded as \texttt{\{SMILES\}}. \\
For the molecule \texttt{\{SMILES\}}, return whether it is an HIV inhibitor or not. \\
From the SMILES \texttt{\{SMILES\}}, predict the binary HIV property. \\
Can you assess whether \texttt{\{SMILES\}} corresponds to an HIV inhibitor? \\
What is the HIV property classification for the compound \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{HIV inhibitor classification prompt template.}
\label{tab:prompts_hiv}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{IUPAC to SMILES Prompt Variants} \\
\midrule
Convert the following IUPAC name to its SMILES representation: \texttt{\{IUPAC\}} \\
What is the SMILES string for the compound named \texttt{\{IUPAC\}}? \\
Generate the canonical SMILES corresponding to the IUPAC name: \texttt{\{IUPAC\}} \\
Given the IUPAC name \texttt{\{IUPAC\}}, return its SMILES notation. \\
Translate this chemical IUPAC name into SMILES format: \texttt{\{IUPAC\}} \\
Can you provide the SMILES representation of \texttt{\{IUPAC\}}? \\
Find the SMILES encoding for the molecule with IUPAC name: \texttt{\{IUPAC\}} \\
I have the IUPAC name \texttt{\{IUPAC\}}. What's the equivalent SMILES string? \\
Please output the SMILES structure that matches this IUPAC name: \texttt{\{IUPAC\}} \\
From the IUPAC name \texttt{\{IUPAC\}}, generate the corresponding SMILES string. \\
\bottomrule
\end{tabular}
\caption{IUPAC-to-SMILES prompt templates.}
\label{tab:prompts_i2s}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{SMILES to IUPAC Prompt Variants} \\
\midrule
Convert the following SMILES string into its IUPAC name: \texttt{\{SMILES\}} \\
What is the IUPAC name for the molecule with SMILES: \texttt{\{SMILES\}}? \\
Generate the IUPAC name corresponding to this SMILES: \texttt{\{SMILES\}} \\
Given the SMILES \texttt{\{SMILES\}}, return its official IUPAC name. \\
Translate this SMILES notation into an IUPAC chemical name: \texttt{\{SMILES\}} \\
Can you provide the IUPAC nomenclature for the compound \texttt{\{SMILES\}}? \\
Find the systematic IUPAC name of the molecule represented by \texttt{\{SMILES\}}. \\
I have the SMILES \texttt{\{SMILES\}}. What's the equivalent IUPAC name? \\
Please output the IUPAC chemical name that matches this SMILES: \texttt{\{SMILES\}} \\
From the SMILES \texttt{\{SMILES\}}, generate the corresponding IUPAC name. \\
\bottomrule
\end{tabular}
\caption{SMILES-to-IUPAC prompt templates.}
\label{tab:prompts_s2i}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Molecule Captioning Prompt Variants} \\
\midrule
Given the SMILES \texttt{\{SMILES\}}, provide a detailed description of the molecule, including its key structural features. \\
Describe the molecular structure represented by the SMILES \texttt{\{SMILES\}} using clear chemical terminology. \\
Write a comprehensive chemical description of the molecule encoded as \texttt{\{SMILES\}}. \\
Based on the SMILES \texttt{\{SMILES\}}, explain the molecule’s functional groups, ring systems, and overall structure. \\
You are an expert chemist. Describe the molecule represented by \texttt{\{SMILES\}} in detail. \\
Provide a detailed molecular caption for the compound specified by the SMILES \texttt{\{SMILES\}}. \\
From the SMILES notation \texttt{\{SMILES\}}, generate a thorough description of the molecule’s chemical characteristics. \\
Explain the structure and notable chemical features of the molecule defined by \texttt{\{SMILES\}}. \\
Using chemical knowledge, describe the molecule represented by the SMILES \texttt{\{SMILES\}}, highlighting important substructures. \\
Produce a detailed, text-based molecular description for the compound encoded as \texttt{\{SMILES\}}. \\
\bottomrule
\end{tabular}
\caption{Molecule captioning prompt templates.}
\label{tab:prompts_caption}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{ESOL Regression Prompt Variants} \\
\midrule
Predict the aqueous solubility (ESOL) value for the molecule with SMILES: \texttt{\{SMILES\}} \\
What is the solubility of \texttt{\{SMILES\}} in water? \\
Estimate the ESOL property of \texttt{\{SMILES\}}. \\
Given the SMILES \texttt{\{SMILES\}}, compute its solubility value. \\
How soluble is \texttt{\{SMILES\}} in water? \\
Report the predicted ESOL value for \texttt{\{SMILES\}}. \\
For the molecule \texttt{\{SMILES\}}, return its solubility estimate. \\
From the SMILES \texttt{\{SMILES\}}, predict the ESOL property. \\
Provide the aqueous solubility for the structure \texttt{\{SMILES\}}. \\
What is the predicted ESOL value for \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{ESOL regression prompt template.}
\label{tab:prompts_esol}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{FreeSolv Regression Prompt Variants} \\
\midrule
Predict the hydration free energy (FreeSolv) for the molecule with SMILES: \texttt{\{SMILES\}} \\
What is the hydration free energy of \texttt{\{SMILES\}}? \\
Estimate the FreeSolv value for \texttt{\{SMILES\}}. \\
Given the SMILES \texttt{\{SMILES\}}, compute its solvation free energy. \\
How favorable is hydration for \texttt{\{SMILES\}}? \\
Report the predicted FreeSolv property for \texttt{\{SMILES\}}. \\
For the molecule \texttt{\{SMILES\}}, return its hydration free energy. \\
From the SMILES \texttt{\{SMILES\}}, predict the FreeSolv value. \\
Provide the solvation free energy for the compound \texttt{\{SMILES\}}. \\
What is the hydration free energy of \texttt{\{SMILES\}} in water? \\
\bottomrule
\end{tabular}
\caption{FreeSolv regression prompt template.}
\label{tab:prompts_freesolv}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Lipo Regression Prompt Variants} \\
\midrule
Predict the lipophilicity (Lipo) value for the molecule with SMILES: \texttt{\{SMILES\}} \\
What is the logD/lipophilicity of \texttt{\{SMILES\}}? \\
Estimate the lipophilicity property of \texttt{\{SMILES\}}. \\
Given the SMILES \texttt{\{SMILES\}}, compute its lipophilicity. \\
How lipophilic is \texttt{\{SMILES\}}? \\
Report the predicted Lipo value for \texttt{\{SMILES\}}. \\
For the molecule \texttt{\{SMILES\}}, return its lipophilicity score. \\
From the SMILES \texttt{\{SMILES\}}, predict the Lipo property. \\
Provide the lipophilicity index for the compound \texttt{\{SMILES\}}. \\
What is the predicted lipophilicity (Lipo) of \texttt{\{SMILES\}}? \\
\bottomrule
\end{tabular}
\caption{Lipophilicity regression prompt template.}
\label{tab:prompts_lipo}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Polymer Oxygen Permeability Prompt Variants} \\
\midrule
Predict the oxygen permeability (in Barrer) of the polymer with SMILES: \texttt{\{SMILES\}}. \\
What is the O$_2$ permeability (Barrer) of the polymer \texttt{\{SMILES\}}? \\
Given the polymer SMILES \texttt{\{SMILES\}}, predict its oxygen permeability expressed in Barrer. \\
Estimate the oxygen permeability of \texttt{\{SMILES\}} in Barrer units. \\
Based on solution--diffusion transport behavior, predict the O$_2$ permeability (Barrer) of the polymer \texttt{\{SMILES\}}. \\
For gas separation membrane applications, predict the oxygen permeability (Barrer) of the polymer \texttt{\{SMILES\}}. \\
Predict the oxygen permeability value (Barrer) for the polymer with SMILES \texttt{\{SMILES\}}. \\
Determine the oxygen permeability coefficient, reported in Barrer, for the polymer \texttt{\{SMILES\}}. \\
Predict the oxygen permeability of the polymer \texttt{\{SMILES\}}. Output a single numeric value in Barrer. \\
Return the oxygen permeability (Barrer) for the polymer represented by \texttt{\{SMILES\}}. \\
\bottomrule
\end{tabular}
\caption{Polymer oxygen permeability regression prompt template.}
\label{tab:prompts_polymer_o2}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Stoichiometric Coefficient Balancing Prompt Variants} \\
\midrule
Balance the following equation by finding the missing coefficient: \texttt{\{EQUATION\}} \\
What coefficient should go in front of \texttt{\{SPECIES\}} to balance \texttt{\{EQUATION\}}? \\
Complete the stoichiometry: fill in the missing coefficient in \texttt{\{EQUATION\}}. \\
For the reaction \texttt{\{EQUATION\}}, what is the correct stoichiometric coefficient of \texttt{\{SPECIES\}}? \\
Find the integer coefficient that balances the molecule \texttt{\{SPECIES\}} in \texttt{\{EQUATION\}}. \\
In the equation \texttt{\{EQUATION\}}, determine the missing multiplier for \texttt{\{SPECIES\}}. \\
What value should replace the blank to balance the equation: \texttt{\{EQUATION\}}? \\
Balance this reaction by supplying the missing number in front of \texttt{\{SPECIES\}}: \texttt{\{EQUATION\}} \\
For \texttt{\{EQUATION\}}, calculate the correct coefficient of \texttt{\{SPECIES\}}. \\
Fill in the missing stoichiometric number in \texttt{\{EQUATION\}}. \\
\bottomrule
\end{tabular}
\caption{Stoichiometric coefficient balancing prompt template.}
\label{tab:prompts_coeff_balancing}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Reaction Yield Prediction Prompt Variants} \\
\midrule
Given the balanced equation \texttt{\{EQUATION\}}, if \texttt{\{MASS\}} of \texttt{\{GIVEN\}} is present, how much \texttt{\{ASKED\}} will form? \\
For the reaction \texttt{\{EQUATION\}}, calculate the required amount of \texttt{\{ASKED\}} if \texttt{\{MASS\}} of \texttt{\{GIVEN\}} is used. \\
In the balanced chemical equation \texttt{\{EQUATION\}}, determine the quantity of \texttt{\{ASKED\}} corresponding to \texttt{\{MASS\}} of \texttt{\{GIVEN\}}. \\
If \texttt{\{MASS\}} of \texttt{\{GIVEN\}} reacts in \texttt{\{EQUATION\}}, what is the yield of \texttt{\{ASKED\}}? \\
Using the balanced equation \texttt{\{EQUATION\}}, find the number of moles of \texttt{\{ASKED\}} that react with \texttt{\{MASS\}} of \texttt{\{GIVEN\}}. \\
For \texttt{\{EQUATION\}}, compute the mass of \texttt{\{ASKED\}} produced when \texttt{\{MASS\}} of \texttt{\{GIVEN\}} is available. \\
According to \texttt{\{EQUATION\}}, how many moles of \texttt{\{ASKED\}} correspond to \texttt{\{MASS\}} of \texttt{\{GIVEN\}}? \\
Using stoichiometry from \texttt{\{EQUATION\}}, calculate the amount of \texttt{\{ASKED\}} from \texttt{\{MASS\}} of \texttt{\{GIVEN\}}. \\
Based on the balanced equation \texttt{\{EQUATION\}}, if \texttt{\{MASS\}} of \texttt{\{GIVEN\}} is consumed, what is the resulting amount of \texttt{\{ASKED\}}? \\
In \texttt{\{EQUATION\}}, find the stoichiometric equivalent of \texttt{\{ASKED\}} when \texttt{\{MASS\}} of \texttt{\{GIVEN\}} is given. \\
\bottomrule
\end{tabular}
\caption{Reaction yield prediction prompt template.}
\label{tab:prompts_yield}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Molecular Weight Prompt Variants} \\
\midrule
Calculate exactly the molecular weight for the compound \texttt{\{SMILES\}}. \\
What is the exact molar mass of \texttt{\{SMILES\}}? \\
Determine the molecular weight corresponding to \texttt{\{SMILES\}}. \\
Find the molecular weight of the molecule with SMILES \texttt{\{SMILES\}}. \\
Compute the molecular weight of \texttt{\{SMILES\}} in Daltons. \\
How heavy is the molecule \texttt{\{SMILES\}} in Daltons? \\
What is the MW (g/mol) for \texttt{\{SMILES\}}? \\
Report the molecular weight of the structure \texttt{\{SMILES\}}. \\
Provide the molar mass of the compound encoded as \texttt{\{SMILES\}}. \\
For the SMILES \texttt{\{SMILES\}}, return its molecular weight. \\
\bottomrule
\end{tabular}
\caption{Molecular weight prediction prompt template.}
\label{tab:prompts_mol_weight_a}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Forward Reaction Prediction Prompt Variants} \\
\midrule
Reactants: \texttt{\{REACTANTS\}} \\
Products: \\
Given the following reactants: \texttt{\{REACTANTS\}}. Predict the reaction products. \\
Consider the chemical reaction involving the reactants \texttt{\{REACTANTS\}}. What products are formed? \\
For the reaction starting from reactants \texttt{\{REACTANTS\}}, determine the resulting products. \\
Based on the listed reactants (\texttt{\{REACTANTS\}}), predict the products of the reaction. \\
In the chemical transformation where the reactants are \texttt{\{REACTANTS\}}, what compounds are produced? \\
Using the given reaction specification:\ Reactants: \texttt{\{REACTANTS\}}\ Identify the products. \\
Determine the products formed when the reactants \texttt{\{REACTANTS\}} undergo reaction. \\
What are the expected reaction products from the reactants \texttt{\{REACTANTS\}}? \\
From the reaction defined solely by the reactants \texttt{\{REACTANTS\}}, predict the products. \\
\bottomrule
\end{tabular}
\caption{Forward reaction prediction prompt template. Reactants are provided and the model is tasked with predicting the corresponding products.}
\label{tab:prompts_forward_reaction}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Retrosynthesis Prompt Variants} \\
\midrule
Products: \texttt{\{PRODUCTS\}} \\
Reactants: \\
Given the following products: \texttt{\{PRODUCTS\}}. Predict the reactants required for their synthesis. \\
Consider the target products \texttt{\{PRODUCTS\}}. What reactants would be used to synthesize them? \\
For the chemical transformation leading to products \texttt{\{PRODUCTS\}}, determine the necessary reactants. \\
Based on the listed products (\texttt{\{PRODUCTS\}}), predict the reactants involved in their formation. \\
In the retrosynthetic analysis of products \texttt{\{PRODUCTS\}}, what reactants are required? \\
Using the given reaction specification:\ Products: \texttt{\{PRODUCTS\}}\ Identify the reactants. \\
Determine the reactants that could give rise to the products \texttt{\{PRODUCTS\}}. \\
What reactants would produce the products \texttt{\{PRODUCTS\}} in a chemical reaction? \\
From the reaction defined by the products \texttt{\{PRODUCTS\}}, predict the corresponding reactants. \\
\bottomrule
\end{tabular}
\caption{Retrosynthetic reaction prediction prompt template. Products are provided and the model is tasked with inferring plausible reactants.}
\label{tab:prompts_retro_reaction}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Representation Equivalence Prompt Variants} \\
\midrule
Do the two chemical representations \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}} describe the same molecule? \\
Determine whether \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}} refer to the same chemical compound. \\
Are \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}} equivalent representations of the same molecule? \\
Do \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}} correspond to the same molecular structure? \\
Is the molecule described by \texttt{\{REP\_A\}} identical to the one described by \texttt{\{REP\_B\}}? \\
Assess whether \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}} denote the same chemical substance. \\
Do these two representations, \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}}, describe the same molecule? \\
Are the chemical entities represented by \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}} the same? \\
Verify whether \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}} correspond to an identical molecule. \\
Given \texttt{\{REP\_A\}} and \texttt{\{REP\_B\}}, determine if they describe the same molecular structure. \\
\bottomrule
\end{tabular}
\caption{Representation equivalence prompt template.}
\label{tab:prompts_rep_equiv}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Chemical Similarity Prompt Variants} \\
\midrule
Which molecule is more chemically similar to \texttt{\{QUERY\}}: \texttt{\{A\}} or \texttt{\{B\}}? \\
Between \texttt{\{A\}} and \texttt{\{B\}}, which is more similar in structure to \texttt{\{QUERY\}}? \\
Determine whether \texttt{\{A\}} or \texttt{\{B\}} is more chemically similar to \texttt{\{QUERY\}}. \\
Which compound more closely resembles \texttt{\{QUERY\}}: \texttt{\{A\}} or \texttt{\{B\}}? \\
Assess the chemical similarity of \texttt{\{A\}} and \texttt{\{B\}} to \texttt{\{QUERY\}}. Which is more similar? \\
Which molecule shares greater structural similarity with \texttt{\{QUERY\}}, \texttt{\{A\}} or \texttt{\{B\}}? \\
Compare \texttt{\{A\}} and \texttt{\{B\}} to \texttt{\{QUERY\}}. Which is more chemically similar? \\
Identify which molecule is more similar to \texttt{\{QUERY\}}: \texttt{\{A\}} or \texttt{\{B\}}. \\
Between the two options, \texttt{\{A\}} and \texttt{\{B\}}, which better matches \texttt{\{QUERY\}} chemically? \\
Given \texttt{\{QUERY\}}, select the molecule that is more chemically similar: \texttt{\{A\}} or \texttt{\{B\}}. \\
\bottomrule
\end{tabular}
\caption{Chemical similarity comparison prompt template.}
\label{tab:prompts_chem_similarity}
\end{table}

\begin{table}[h]
\centering
\small
\begin{tabular}{p{0.95\linewidth}}
\toprule
\textbf{Property (Weight) Comparison Prompt Variants} \\
\midrule
Which molecule has a \texttt{\{DIR\}} \texttt{\{PROPERTY\}}, \texttt{\{A\}} or \texttt{\{B\}}? \\
Determine whether \texttt{\{A\}} or \texttt{\{B\}} has the \texttt{\{DIR\}} value of \texttt{\{PROPERTY\}}. \\
Between \texttt{\{A\}} and \texttt{\{B\}}, which exhibits a \texttt{\{DIR\}} \texttt{\{PROPERTY\}}? \\
Which compound shows a \texttt{\{DIR\}} \texttt{\{PROPERTY\}}: \texttt{\{A\}} or \texttt{\{B\}}? \\
Assess the \texttt{\{PROPERTY\}} of \texttt{\{A\}} and \texttt{\{B\}}. Which one is \texttt{\{DIR\}}? \\
Identify whether \texttt{\{A\}} or \texttt{\{B\}} has the \texttt{\{DIR\}} \texttt{\{PROPERTY\}}. \\
Compare \texttt{\{A\}} and \texttt{\{B\}} in terms of \texttt{\{PROPERTY\}}. Which is \texttt{\{DIR\}}? \\
Which molecule demonstrates a \texttt{\{DIR\}} value for \texttt{\{PROPERTY\}}, \texttt{\{A\}} or \texttt{\{B\}}? \\
For the property \texttt{\{PROPERTY\}}, which molecule is \texttt{\{DIR\}}: \texttt{\{A\}} or \texttt{\{B\}}? \\
Given \texttt{\{A\}} and \texttt{\{B\}}, determine which has the \texttt{\{DIR\}} \texttt{\{PROPERTY\}}. \\
\bottomrule
\end{tabular}
\caption{Pairwise property comparison prompt template (e.g., molecular weight, solubility).}
\label{tab:prompts_property_comparison}
\end{table}


==> tables/reg_r2.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model} & \textbf{ESOL $R^2$} & \textbf{Lipo $R^2$} & \textbf{FreeSolv $R^2$} \\
        \midrule
        ChemLLM            & 0.6673 & -1.2114 & -111.7115 \\
        ChemDFM            & 0.6550 & -1.2498 & -60.9002 \\
        Chemr              & 0.6458 & -1.2559 & -111.3903 \\
        General-Reasoner   & 0.6252 & -1.2453 & -112.4126 \\
        Falcon             & 0.6416 & -1.1832 & -112.1851 \\
        Galatica           & 0.6520 & -1.2518 & -110.5977 \\
        Qwen2              & 0.6258 & -1.1962 & -18.5671 \\
        Qwen3              & 0.6364 & -1.2256 & -112.3573 \\
        Mistral            & 0.6597 & -1.2159 & -109.9610 \\
        Gemma2             & 0.6415 & -1.1710 & -109.9393 \\
        Gemma3             & 0.6451 & -1.2152 & -110.9743 \\
        Llama2             & 0.6362 & -1.1981 & -64.0810 \\
        Llama3             & 0.6342 & -1.2342 & -110.1538 \\
        Deepseek-r1        & 0.6435 & -1.1909 & -110.0071 \\
        GPT-4o             & 0.6316 & -1.2624 & -110.9038 \\
        GPT-4.1            & 0.6201 & -1.1890 & -111.3937 \\
        GPT-5              & 0.6313 & -1.2207 & -61.5769 \\
        \bottomrule
    \end{tabular}
    \vspace{6px}
    \caption{Coefficient of determination ($R^2$) for ESOL, Lipo, and FreeSolv regression tasks across evaluated models.}
    \label{tab:r2_regression_results}
\end{table}

==> tables/subset_split_full.tex <==
\begin{table*}[]
    \centering
    \resizebox{0.8\textwidth}{!}{
        \begin{tabular}{|c|c|c|c|}
            \hline
            Task Type & Subtask & Full Test Count & Subset in ChemDIRT \\
            \hline \hline
            Description & Carbon Count & Ours & 100 \\
            & Ring Count & Ours & 100 \\
            & Functional Group Presence & Ours & 100 \\
            & Bond Type Presence & Ours & 100 \\
            \hline
            Classification & BACE & 151 & 151 \\
            & BBBP & 203 & 203 \\
            & ClinTox & 148 & 148 \\
            & HIV & 4113 & 100 \\
            \hline
            Design & IUPAC2SMILES & Ours & 100 \\
            & SMILES2IUPAC & Ours & 100 \\
            & Photo2SMILES & Ours & 100 \\
            & Photo2IUPAC & Ours & 100 \\
            & Text-Description Generation & 100 & 100 \\
            \hline
            Analytical & RAG-based QA & 211 & 211 \\
            & T/F w/Explanation & 100 & 100 \\
            & Open Response & 100 & 100 \\
            \hline
            Regression & ESOL & 113 & 113 \\
            & Lipophilicity & 420 & 420 \\
            & FreeSolv & 65 & 65 \\
            & O2 & 179 & 179 \\
            \hline
            Computational & Physical Unit Calculation & 500 & 392 \\
            & Coefficient Balancing & 500 & 100 \\
            & Yield Prediction & 300 & 300 \\
            & Molecular Weight Calculation & Ours & 100 \\
            \hline
            Mechanistic & Forward Reaction Prediction (SMILES) & 100 & 100 \\
            & Forward Reaction Prediction (Formula) & Ours & 100 \\
            & Forward Reaction Prediction (Photo) & Ours & 100 \\
            & Retrosynthesis Planning (SMILES) & 100 & 100 \\
            & Retrosynthesis Planning (Formula) & Ours & 100 \\
            & Retrosynthesis Planning (Photo) & Ours & 100 \\
            \hline
            Relational & Representation Equivalence & Ours & 100 \\
            & Chemical Similarity Validation & Ours & 100 \\
            & Molar Weight Comparison & Ours & 100 \\
            \hline
        \end{tabular}
    }
    \caption{Task Counts and Subset Size}
    \label{tab:subset_split_full}
\end{table*}



==> tables/subset_split_short.tex <==
\begin{table}[]
    \centering
    \resizebox{0.8\textwidth}{!}{
        \begin{tabular}{|c|c|}
            \hline
            Task Type & Count \\
            \hline \hline
            Description & 400 \\
            \hline
            Classification & 605 \\
            \hline
            Design & 300 \\
            \hline
            Analytical & 536 \\
            \hline
            Regression & 658 \\
            \hline
            Computational & 819 \\
            \hline
            Mechanistic & 400 \\
            \hline
            Relational & 300 \\
            \hline
        \end{tabular}
    }
    \caption{Task Counts and Subset Size}
    \label{tab:subset_split}
\end{table}


